Extending ALCQIO with reachability

We introduce a description logic ALCQIO_{b,Re} which adds reachability assertions to ALCQIO, a sub-logic of the two-variable fragment of first order logic with counting quantifiers. ALCQIO_{b,Re} is well-suited for applications in software verification and shape analysis. Shape analysis requires expressive logics which can express reachability and have good computational properties. We show that ALCQIO_{b,Re} can describe complex data structures with a high degree of sharing and allows compositions such as list of trees. We show that the finite satisfiability and implication problems of ALCQIO_{b,Re}-formulae are polynomial-time reducible to finite satisfiability of ALCQIO-formulae. As a consequence, we get that finite satisfiability and finite implication in ALCQIO_{b,Re} are NEXPTIME-complete. Description logics with transitive closure constructors have been studied before, but ALCQIO_{b,Re} is the first description logic that remains decidable on finite structures while allowing at the same time nominals, inverse roles, counting quantifiers and reachability assertions,

==> app-program-analysis.tex <==


%00000000000000000000000000000000000000
%00000000000000000000000000000000000000
%00000000000000000000000000000000000000
%00000000000000000000000000000000000000

\global\long\def\SL{\mathrm{\mathbf{SL}}}
\global\long\def\SLls{\mathrm{\mathbf{SL{\scriptstyle ls}}}}
%\global\long\def\SLind{\mathrm{\mathbf{SL{\scriptstyle ind}}}}
\global\long\def\nil{\mathrm{null}}
\global\long\def\tree{\mathrm{tree}}
\global\long\def\lss{\mathrm{list-of-lists}}
\global\long\def\ls{\mathrm{ls}}
%\global\long\def\iffdef{\stackrel{\mathrm{{\scriptstyle def}}}{\mathrm{iff}}}
\global\long\def\iffdef{\mathrm{iff}}
\global\long\def\arrowfin{\stackrel{\mathrm{{\scriptscriptstyle fin}}}{\mathrm{\to}}}
\global\long\def\false{\mathbf{F}}
\global\long\def\true{\mathbf{T}}
\global\long\def\emp{\mathrm{emp}}
\global\long\def\NR{\mathsf{N_{R}}}
\global\long\def\NRF{\mathsf{N_{F}}}
\global\long\def\NC{\mathsf{N_{C}}}
\global\long\def\NCshp{\mathsf{N_{C}^{shp}}}
\global\long\def\NCdom{\mathsf{N_{C}^{dom}}}
\global\long\def\NI{\mathsf{N_{I}}}
\global\long\def\NIdom{\mathsf{N_{I}^{dom}}}
\global\long\def\NIvar{\mathsf{N_{I}^{var}}}
\global\long\def\NIloc{\mathsf{N_{I}^{free}}}
\global\long\def\lb{[\![}
\global\long\def\rb{]\!]}
\global\long\def\bv{\,\brokenvert\:}
\global\long\def\mm{\mathcal{M}}
\global\long\def\nn{\mathcal{N}}
\global\long\def\abo{\mbox{abort}}
\global\long\def\mmdom{M}
\global\long\def\sM{\mathscr{s}(\mm)}
\global\long\def\tm{\tau_{m}}
\global\long\def\tauField{\tau_{\mathrm{fields}}}
%\global\long\def\tauFree{\tau_{\mathrm{free}}}
\global\long\def\tauVar{\tau_{\mathrm{var}}}
\global\long\def\eqqm{\stackrel{{\scriptscriptstyle ?}}{=}}
\global\long\def\bigsqcap{\sqcap}
\global\long\def\L{\mathcal{L}}
\global\long\def\DL{\mathcal{ALCHOIQ}br}
\global\long\def\err{\mbox{err}}
\global\long\def\FO{\mathrm{FO}}

\newcommand{\Addr}{Addresses}
\newcommand{\nncur}{\nn_{cur}}
\newcommand{\nngho}{\nn_{gho}}
\newcommand{\mmcur}{\mm_{cur}}
\newcommand{\mmgho}{\mm_{gho}}
\newcommand{\gho}{{gho}}
%\newcommand{\exttau}{\tau_{ext}}
\newcommand{\MemPool}{MemPool}
\newcommand{\annot}{{annot}}
\newcommand{\sannot}{{shp}}
\newcommand{\vercond}{{vercond}}
\newcommand{\control}{{ctrl}}
%\newcommand{\nn}{\mathcal{N}}
\newcommand{\pp}{\mathcal{P}}
\renewcommand{\ll}{LL}
\newcommand{\pre}{{pre}}
\newcommand{\post}{{post}}
\newcommand{\LLPrograms}{LLPrograms}
\newcommand{\linit}{\ell_{init}}
\newcommand{\Init}{Init}




\newif\ifCont
\Conttrue

\ifCont
\newcommand{\dmnCnt}{cnt}
\newcommand{\domainContent}{content}
\newcommand{\DomainContent}{Content}
\else
\newcommand{\dmnCnt}{dmn}
\newcommand{\domainContent}{domain}
\newcommand{\DomainContent}{Domain}
\fi

\section{Application to program analysis}

\subsection{Memory Structures \label{subse:structures--1}\label{subse:memory-structures--1}}

We use ordinary first order structures to represent memory in a
precise way. A \emph{structure} (or, \emph{interpretation}) is a tuple
$\mm=(M,\tau,\cdot)$, where
(i) $M$ is an infinite set (the \emph{universe}),
(ii) $\tau$ is a set of \emph{constants} and \emph{relation symbols}
  with an associated non-negative arity, and
(iii) $\cdot$ is an \emph{interpretation function}, which assigns to
  each constant $c\in \tau$ an element $c^\mm\in M$, and to each
  $n$-ary relation symbol $R\in \tau$ an $n$-ary relation $R^{\mm}$
  over $M$. Each relation is either unary or binary
  (i.e. $n\in\{1,2\}$).
  Given $A\subseteq M$, a binary $R^\mm$, $R^\mm$ and $e\in A^\mm$, we may use the notation
  $R^\mm(e)$ if $R^\mm$ is known to be a function over $A^\mm$.

A {\em Memory structure} describes a snapshot of the heap and the
local variables. We assume sets
$\tauVar\subseteq \tau$ of constants $\tauField\subseteq \tau$ of
binary relation symbols.  We will later employ these symbols for
variables and fields in programs.  A {\em memory structure} is a structure
$\mm=(M,\tau,\cdot)$ that satisfies the following conditions:
\begin{enumerate}[(1)]
\item % $\tauVar\cup \tauField\subseteq \tau$ and
  $\tau$ includes the constants $o_{\nil}$, $o_\true$, $o_\false$.
\item $\tau$ has the unary relations $\Addr$, $Alloc$, $PossibleTargets$, $\MemPool$,
  and $Aux$.
\item $Aux^\mm=\{o_\nil^\mm,o_\true^\mm,o_\false^\mm\}$ and $|Aux^\mm|=3$.
\item $\Addr^\mm\cap Aux^\mm= \emptyset$ and $\Addr^\mm \cup Aux^\mm =
  M$.
\item $Alloc^\mm$, $PossibleTargets^\mm$ and $\MemPool^\mm$ form a partition of $\Addr^\mm$.
\item $c^\mm\in M\backslash \MemPool^\mm$ for every constant $c$ of $\tau$.
\item For all $f\in  \tauField$, $f^\mm$ is a function from
  $\Addr^\mm$ to $M\backslash \MemPool^\mm$.
\item If $e\in \MemPool^\mm$, then $f^\mm(e)\in \{o_\nil^\mm,o_\false^\mm\}$.
\item $R^{\mm}\subseteq (M\backslash \MemPool^\mm)^n$ for every\footnote{Here $n\in \{1,2\}$.}
  $n$-ary $R\in \tau \setminus (\{\MemPool \}\cup \tauField)$.
 \item $Alloc^\mm$ and $PossibleTargets^\mm$  are finite. $\MemPool^\mm$ is infinite.

\end{enumerate}

We explain the intuition behind memory structures. Variables in
programs will either have a Boolean value or be pointers. Thus, to
represent $\nil$ and the Boolean values $\true$ and $\false$, we
employ the auxiliary relation $Aux^\mm$ storing 3 elements
corresponding to the 3 values. $\Addr^{\mm}$ represents the memory
cells.
The relation $Alloc^\mm$ is the set of allocated
cells, $PossibleTargets^\mm$ contains all cells which are not allocated,
but are pointed to by allocated cells (for technical reasons it possibly contains some other unallocated cells).
$\MemPool^\mm$ contains the cells which are not allocated, do
not have any field values other than $\nil$ and $\false$, are not
pointed to by any field, do not participate in any other relation and
do not interpret any constant (see (6-9)). The memory cells in $\MemPool$ are
the candidates for allocation during the run of a program.
 Since the allocated memory should by finite at any point of the
execution of a program, we require that
$Alloc^\mm $ and $PossibleTargets^\mm$
are finite (see (10)), while the available memory $\Addr^\mm$ and the memory pool $\MemPool^\mm $
are infinite. Finally, each
cell is seen as a record with the fields of
$\tauField$.


\subsubsection{Ghost symbols}
As discussed in Section \ref{se:EPM-example-DL},
in order to allow invariants of the form
$
\begin{array}{lll}
 \varphi_{lists-updt} &=& ELst_{\gho} \equiv ELst  \land
  PLst_{\gho}\sqcup o_{proj}  \equiv  PLst
\end{array}
$\\
we need ghost symbols.
We assume $\tau$ contains, for every symbol e.g. $s \in \tau$, the symbol $s_{\gho}$.
Therefore, memory structures actually contain {\em two}
snapshots of the memory:
one is the {\em current} snapshot, on which the program operates,
and the other is a {\em ghost} snapshot, which is a snapshot of the memory
 at the beginning of the program, and which the program does not change or interact with.
We denote the two underlying memory structures of $\mm$ by
$\mmcur$ and $\mmgho$.
Since the interpretations of ghost symbols should not change throughout the run of a program,
they will sometime require special treatment.

\subsection{Syntax and Semantics of the Programming Language }

\subsubsection{Loopless Programs}
are generated by the following syntax:
\begin{center}
$
\begin{array}{lll}
e & :: & var.f\mid var\mid\nil\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,(f\in\tauField,\, o_{var}\in\tauVar)\\
b & :: &(e_{1}=e_{2})\mid\,\sim b\mid(b_{1}\, and\, b_{2})\mid(b_{1}\, or\, b_{2}) \mid \true \mid \false\\
S & :: & var_{1}:=e_{2}\mid var_{1}.f:=e_{2}\mid skip\mid S_{1};S_{2}
\mid var:=new \mid dispose(var)  \mid \\
 & & if\,\, b\,\, then\,\, S_{1}\,\, fi
  \mid if\,\, b\,\, then\,\, S_{1}\,\, else\,\, S_{2}\,\, fi \mid assume(b)
\end{array}
$
\end{center}
 %We denote by $Variables$ and $Fields$ the corresponding sets of
%names and by
 Let $Exp$
denote the set of expressions $e$ and $Bool$ denote the set of Boolean
expressions $b$.
To define the semantics of pointer and Boolean expressions, we extend  $f^{\mm}$
by $f^{\mm}(\err)=\err$ for every $f\in \tauField$. We define
$\mathcal{E}_e(\mm):Exp\,\,\to \Addr^\mm\cup\{\nil,\err\}$ and $\mathcal{B}_b(\mm):Bool\to\{o_\true,o_\false,\err\}$
(with $\err\not\in M$):
\begin{center}
$
\begin{array}{llll}
\mathcal{E}_{var}(\mm) & =o_{var}^{\mm},  \mbox{ if }o_{var}^{\mm}\in Alloc^{\mm}\ &
\mathcal{B}_{e_{1}=e_{2}}(\mm) & =\err  \mbox{ if }\mathcal{E}_{e_{i}}(\mm)=\err, i\in\{1,2\}\\
\mathcal{E}_{var}(\mm) & =\err,  \mbox{ if }o_{var}^{\mm}\not\in Alloc^{\mm}&
\mathcal{B}_{e_{1}=e_{2}}(\mm) & =o_\true,  \mbox{ if }\mathcal{E}_{e_{1}}(\mm)=\mathcal{E}_{e_{2}}(\mm)\\
\mathcal{E}_{ar.f}(\mm) &=f^{\mm}(\mathcal{E}_{var}(\mm))&
\mathcal{B}_{e_{1}=e_{2}}(\mm) & =o_\false,  \mbox{ if }\mathcal{E}_{e_{1}}(\mm)\not=\mathcal{E}_{e_{2}}(\mm)
\end{array}
$\end{center}
$\mathcal{B}$ extends naturally w.r.t. the Boolean connectives.

The operational semantics of the programming language is:
For any command $S$, if $\mathcal{E}$ or $\mathcal{B}$
give the value $\err$, then $\left\langle S,\mm\right\rangle \leadsto\abo$.
Otherwise, the semantics is as listed below.
First we assume that
in the memory structures involved
all relation symbols either belong to $\tauField$, are ghost symbols
or are the required symbols of memory structures ($Alloc$, $Aux$, etc.).
\begin{enumerate}
\item $\left\langle skip,\mm\right\rangle \leadsto\mm$.
\item %If $\mathcal{E}\lb e_{2}\rb(\mm)]=\err$, then $\left\langle var_{1}:=e_{2},\mm\right\rangle \leadsto\abo$;\\
%otherwise,
$\left\langle var_{1}:=e_{2},\mm\right\rangle \leadsto[\mm\mid o_{var_{1}}^{\mm}\mbox{ is set to }\mathcal{E}_{e_{2}}(\mm)]$.
\item $\left\langle var:=new,
\mm\right\rangle\leadsto$
$[\mm\mid \mbox{For some }t\in\MemPool^\mm,$ \\$ t\mbox{ is moved to }Alloc^{\mm}\mbox{ and }o_{var}^{\mm}\mbox{ is set to }t],$
\item If $o_{var}^{\mm}\not\in Alloc^{\mm}$, $\left\langle dispose(var),\mm\right\rangle \leadsto\abo$;\\
otherwise $\left\langle dispose(var),\mm\right\rangle \leadsto[\mm\mid o_{var}^{\mm}\mbox{ is removed from }Alloc^{\mm}]$.
\item $\left\langle S_{1};S_{2},\mm\right\rangle \leadsto\left\langle S_{2},\left\langle S_{1},\mm\right\rangle \right\rangle$
\item
$\left\langle if\,\, b\,\, then\,\, S_{\true}\,\, else\,\, S_{\false},\mm\right\rangle \leadsto\left\langle S_{tv},\mm\right\rangle $
where $tv=\mathcal{B}_{b}(\mm)$.
\item
$\left\langle if\,\, b\,\, then\,\, S\,\, ,\mm\right\rangle \leadsto
\left\langle if\,\, b\,\, then\,\, S\,\, else\,\, skip\,\, fi ,\mm\right\rangle$.
\item
If $\mathcal{B}_{b}(\mm)=\true$, then
$\left\langle assume(b), \mm\right\rangle \leadsto \mm$;\\
otherwise $\left\langle assume(b), \mm\right\rangle \leadsto \abo$.
\end{enumerate}
If $\mm$ is
a memory structure and $\left\langle S,\mm\right\rangle \leadsto\mm'$,
then $\mm'$ is a memory structure.

Now consider a relation symbol e.g. $ELst$.
If $\left\langle S,\mm\right\rangle \leadsto\mm'$,
then we want to think of $ELst^{\mm}$ and $ELst^{\mm'}$ as the employee list
before and after the execution of $S$. However, the constraints that
$ELst^{\mm}$ and $ELst^{\mm'}$ are lists and that
$ELst^{\mm'}$ is indeed obtained from from $ELst^{\mm}$ by running $S$
will be expressed as formulae.
In the $\leadsto$ relation, we allow any values for $ELst^\mm$ and $ELst^{\mm'}$.

For any tuple $\bar{R}$ of relation symbols which do not belong to $\tauField$,
are not ghost symbols
and are not the required symbols of memory structures ($Alloc$, $Aux$, etc.),
we extend $\leadsto$ as follows: if $\left\langle S,\mm\right\rangle \leadsto\mm'$,
then $\left\langle S,\left\langle \mm,\bar{R}^{\mm}\right\rangle \right\rangle \leadsto\left\langle\mm',\bar{R}^{\mm'}\right\rangle$,
for any tuples $\bar{R}^{\mm}$ and $\bar{R}^{\mm'}$.


\subsubsection{Programs with Loops} are represented as hybrids of the programming language for loopless code
and control flow graphs.
 \begin{definition}[Program]\label{def:program}
 A {\em program} is $G = \left\langle V, E,\linit, shp, \dmnCnt,\lambda\right\rangle$
 such that
 $G=(V,E)$ is a directed graph with no multiple edge but possibly containing self-loops, $\linit \in V$ has in-degree $0$,
  $shp:V\to \SLls$, $\dmnCnt:V\to \L(\tau)$ are functions, and $\lambda$ is a function from $E$ to the set of loopless programs.
 \end{definition}

\begin{tabular}{ll}
Here is the code $S$ from the introduction:   &
\multirow{5}{*}{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \includegraphics[scale=0.80]{ProgramGraph}}\\
\end{tabular}\\
\begin{tabular}{ll}
$V=\{\ell_{b},\ell_l,\ell_{e}\}$ & $E=\{(\ell_{b},\ell_l),(\ell_l,\ell_l),(\ell_l,\ell_{e})\}$ \\
$\lambda(\ell_{b},\ell_l)=S_{b}$ & $\linit=\ell_{b}$ \\
 $\lambda(\ell_l,\ell_l)=assume(\sim(e\,=\,\nil));S_{\ell_l}$\\
$\lambda(\ell_l,\ell_e)=assume(e\,=\,\nil);S_e$
\end{tabular}
\\ \ \\
$S_{b}$, $S_{\ell_l}$ and $S_{e}$ denote
 the three loopless code blocks which are respectively the code block before the loop, inside the loop and after the loop.
 The annotations $shp$ and $\dmnCnt$ are described in Section \ref{se:general-meth-example}.

The semantics of programs derive from the semantics of loopless programs and is given in terms of program paths.
Given a program $G$, a {\em path in $G$} is a finite sequence of directed edges
$e_1,\ldots,e_t$ such that for all $1\leq i\leq t-1$, the tail of $e_i$
is the head of $e_{i+1}$.
A path may contain cycles.
% We extend the $\leadsto$ relation to paths in programs:
 \begin{definition}[$\leadsto^*$ for paths]
 Given a program $G$, a path $P$ in $G$,
 and memory structures $\mm_1$ and $\mm_2$
 we define whether
 $\left\langle P, \mm_1\right\rangle\leadsto^* \mm_2$
 holds inductively.
 \begin{itemize}
 \item If $P$ is empty, then $\left\langle P, \mm_1\right\rangle\leadsto^* \mm_2$ iff $\mm_1=\mm_2$.
 \item If $e_t$ is the last edge of $P$, then $\left\langle P, \mm_1\right\rangle\leadsto^* \mm_2$ iff
 there is $\mm_3$ such that
 $\left\langle P\backslash\{e_t\}, \mm_1 \right\rangle\leadsto^* \mm_3$
 and $\left\langle \lambda(e_t), \mm_1 \right\rangle\leadsto^* \mm_3$.
  $P\backslash\{e_t\}$ denotes the path obtained from $P$ by removing the last edge $e_t$.
 \end{itemize}
 \end{definition}

\subsection{Hoare-style Proof System}

Now we are ready to state our two-step verification methodology that we formulated in Section \ref{se:intro} precisely.
Our methodology assumes a program $P$ as in Definition~\ref{def:program} as input (ignoring the $shp$ and $\dmnCnt$ functions for the moment).

\textbf{I. Shape Analysis.}
The user annotates the program locations with SL formulae from $\SLls$ (stored in the $shp$ function of $P$).
Then the user proves the validity of the $\SLls$ annotations, for example, by using techniques from~\cite{pr:BCO05}.

\textbf{II. Content Analysis.}
The user annotates the program locations with $\L$-formulae that she wants to verify (stored in the $\dmnCnt$ function of $P$).
We point out that an annotation $\dmnCnt(\ell)$ can use the concepts occurring in $\alpha(shp(\ell))$ (recall that $\alpha: \SLls \rightarrow \L$ maps SL formulae to $\L$-formulae).

In the rest of the paper we discuss how to verify the $\dmnCnt$ annotations.
In Section~\ref{se:methodology} we describe how to derive a verification condition for every program edge.
The verification conditions rely on the backwards propagation function $\Theta$ for $\L$-formulae which we introduce in Section~\ref{se:backwards-example}.
The key point of our methodology is that the validity of the verification conditions can be discharged automatically by a satisfiability solver for $\ctwotree$-formulae.
We show that all the verification conditions are valid if and only if $\dmnCnt$ is inductive.
Intuitively, $\dmnCnt$ being inductive ensures that the annotations $\dmnCnt$ can be used in an inductive proof to show that all reachable memory structures indeed satisfy the annotations $\dmnCnt(\ell)$ at every program location $\ell$ (see Definition~\ref{def:inductive-annotation} below).


%
%For concreteness, we have defined an automatic translation from $\SLls$ annotations to $\L$-formulae in Section \ref{se:expressing-shape-invariants}.
%However, we want to point out that our methodology is independent of the concrete choice of the shape predicates.
%We only require a translation of shape invariants to $\L$-formulae, as discussed in Section \ref{se:expressing-shape-invariants}.
%
%The user translates the shape invariants into $\L$-formulae
%
%For concreteness, we have stated the SL $\SLls$ as a possible language for shape annotations in Section~\ref{se:SLls}.


%Note that $\Psi$ is a that is \emph{precise} for loopless code.


\subsection{Content Verification}\label{se:methodology}

 We want to prove that, for every initial memory structure $\mm_1$
 from which the computation satisfies $shp$ and which satisfies the \domainContent~pre-condition $\dmnCnt(\linit)$,
 the computation satisfies $\dmnCnt$. Here are the corresponding verification conditions, which annotate the vertices of $G$:

\begin{definition}[Verification conditions]
 Given a program $G$, $VC$ is the function from $E$ to $\L$
 given for $e=(\ell_0,\ell)$ by
 \begin{eqnarray*}
    VC(e) &=& \neg \big[ \beta(shp(\ell_0))\land tr(\dmnCnt(\ell_0))  \land tr\left( \Theta_{\lambda(e)}\big(\alpha(shp(\ell)) \land \neg  \dmnCnt(\ell)\big)\right)\big]
 \end{eqnarray*}
 $VC(e)$ {\em holds} if $VC(e)$ is a tautology over memory structures ($\top \models_m VC(e)$).
 %for every extended memory structure $\nn$, tuple of relations $\bar{U}=(U_R : R\in \tau\backslash \tauField)$ and tuple $\bar{d}$ we have
%\[\left\langle \nn, \bar{U}, \bar{d} \right\rangle \models VC(e)\]
% $\bar{U}$ interprets the primed relation symbols in $\tau_{ext,Y}'$.
 \end{definition}
 $\Theta$ is discussed in Section \ref{se:backwards--}. As we will see, $VC(\ell_0,\ell)$ expresses that
 when running the loopless program $\lambda(e)$ when the memory satisfies the the annotations of $\ell_0$,
 and when the shape annotation of $\ell$ is at least partly true (i.e., when $\alpha(shp(\ell))$),
 the content annotation of $\ell$ holds.


 Let $J$ be a set of  memory structures.
 For a formula in $\ctwotree$ or $\L$, we write $J\models\varphi$
 if, for every $\mm\in J$, $\mm\models \varphi$.
 Let $Init$ be a set of memory structures.
 \begin{definition}[Inductive program annotation]
 \label{def:inductive-annotation}
 Let $f:V\to \ctwotree$.
 We say $f$ is {\em inductive} for $Init$ if (i) $Init\models f(\ell_{init})$, and (ii)
 for every edge $e=(\ell_1,\ell_2)\in E$ and memory structures
 $\mm_1$ and $\mm_2$ such that $\mm_1\models f(\ell_1)$ and $\left\langle \lambda(e),\mm_1\right\rangle \leadsto \mm_2$,
 we have $\mm_2\models f(\ell_2)$.

 We say $shp$ is inductive for $Init$ if the composition $shp\circ\beta:V\to\ctwotree$ is inductive for $Init$.


 We say {\em $\dmnCnt$ is inductive for $Init$ relative to $shp$}
 if $shp$ is inductive for $Init$ and
 $g:V\to\ctwotree$ is inductive for $Init$,
 where $g(\ell)=tr(\dmnCnt(\ell))\land \beta(shp(\ell))$.
 \end{definition}

 \vspace{4pt}
 \begin{theorem}[Soundness and Completeness of the Verification Conditions] \label{th:soundness-completeness}
 Let $G$ be a program such that $shp$ is inductive for $Init$ and $Init\models cnt(\ell_{init})$.
The following statements are equivalent:\\
 (i)  For all $e\in E$, $VC(e)$ holds.\ \ \ \ \ (ii)  $\dmnCnt$ is inductive for $Init$ relative to $shp$.
 \end{theorem}

 We make the notion of a computation satisfying the verification conditions precise using the following definition:
 \begin{definition}[$Reach(\ell)$]
 Given a program $G$, a node $\ell\in V$, and a set $\Init$ of memory structures, % such that $(\nn_0)_{cur}=(\nn_{init})_{\gho}$ for each $\nn_0\in \Init$,
 $Reach(\ell)$ is the set of  memory structures $\mm$ for which there is
 $\mm_{init} \in \Init$ and a path $P$ in $G$ starting at $\linit$
 such that $\left\langle P,\mm_{init}\right\rangle\leadsto^* \mm$.
 \end{definition}
 In particular, $Reach(\ell_{init})=Init$.
 The proof of Theorem \ref{th:soundness-completeness} and its consequence Theorem \ref{th:soundness-2} below
 are in Appendix \ref{app:soundness-completeness}.
 \begin{theorem}[Soundness of the Verification Methodology] \label{th:soundness-2}
 Let $G$ be a program such that $shp$ is inductive for $Init$ and $Init\models cnt(\ell_{init})$.
 If for all $e\in E$,
 $VC(e)$ holds, then for $\ell\in V$, $Reach(\ell)\models \dmnCnt(\ell)$.
 \end{theorem}

\subsection{Backwards Propagation and the Running Example}\label{se:backwards--}\label{se:backwards-example}
Here we shortly discuss the backwards propagation of a formula along a loopless program $S$.
Let $\left\langle S, \mm_1\right\rangle\leadsto \mm_2$ where $\mm_1$ and $\mm_2$
are memory structures over the same vocabulary $\tau$.
E.g., in our running example, for $i=1,2$, $\mm_i$ is
\[
\begin{array}{l}
\left\langle M, ELst^{\mm_i}, next^{\mm_i}, mngBy^{\mm_i}, \cdots,\right.
\left. ELst_{\gho}^{\mm_i}, next_{\gho}^{\mm_i},  \cdots, Alloc^{\mm_i}, Aux^{\mm_i} \cdots  \right\rangle
\end{array}
\]

We will show how to translate a formula for $\mm_2$ to a formula for an extended $\mm_1$.
Fields and variables in $\mm_2$ will be translated by the backwards propagation
 into expressions
involving elements of $\mm_1$. For ghost symbols $s_{\gho}$, $s_{\gho}^{\mm_1}$ will be used instead of $s_{\gho}^{\mm_2}$
since they do not change during the run of the program. Let $\tau^{rem}\subseteq \tau$ be the set of the remaining symbols,
i.e.  the symbols of $\tau \setminus (\{PossibleTargets,\MemPool \}\cup \tauField)$ which are not ghost symbols,
for example $ELst$, but not $ELst_{\gho}$, $next$ or $mngBy$.
We need the result of the backwards propagation to refer to the interpretations of symbols in $\tau^{rem}$
from $\mm_2$ rather than $\mm_1$.
Therefore,
these interpretations are copied as they are from $\mm_2$ and added to $\mm_1$ as follows.
For every $R\in \tau^{rem}$, we add a symbol $R^{ext}$ for the copied relation.
We denote by $(\bar{R}^{ext})^{\mm_1}$ the tuple
$
 \big((R^{ext})^{\mm_1} : (R^{ext})^{\mm_1}=R^{\mm_2}\mbox{ and }R\in\tau^{rem}\big)
$
Let $\tau^{ext}$ extend $\tau$ with $R^{ext}$ for each $R\in\tau^{rem}$.
The backwards propagation updates the fields and variables according to the loopless code.
Afterwards, we substitute the symbols $R\in\tau^{rem}$ in $\varphi$ with the corresponding $R^{ext}$.

We present here a somewhat simplified version of the backwards propagation lemma. The precise version is similar in spirit
and is given in Appendix \ref{app:backward}.
\begin{lemma}[Simplified]\label{lem:backwards--} \label{se:backwards-ghost--}
Let $S$ be a loopless program, let
$\mm_1$ and $\mm_2$ be  memory structures, and
 $\varphi$ be an $\L$-formula over $\tau$.
\begin{enumerate}
 \item If $\left\langle S, \mm_1\right\rangle \leadsto \mm_2$,
 then:
 $\mm_2\models \varphi$ iff
$\left\langle \mm_1, (\bar{R}^{ext})^{\mm_1}\right\rangle \models \Theta_{S}(\varphi)$.
\item If $\left\langle S, \mm_1\right\rangle\leadsto \abo$, then
$\left\langle \mm_1, (\bar{R}^{ext})^{\mm_1},\right\rangle \not\models \Theta_{S}(\varphi)$.
\end{enumerate}
\end{lemma}

As an example of the backwards propagation process,
we consider a formula from Section \ref{se:general-meth-example},
which is part of the \domainContent~annotation of $\ell_l$
and perform the backwards propagation on the loopless program inside the loop:
\[
\begin{array}{lll}
\varphi_{p-as-\ell_l} &=&
P_1 \sqcap\exists wrkFor_{\gho}.o_{\nil} \equiv
P_1 \sqcap\exists wrkFor.o_{proj}
\end{array}
\]

Since $next$ does not occur in $\varphi_{p-as-\ell_l}$, backwards propagation of $\varphi_{p-as-\ell_l}$
over $e := e.next$ does not change the formula (however $\alpha(shp(\ell_l))$
by this command). The backwards propagation of the $if$ command gives
\[
\begin{array}{ll}
 \Psi_{S_{\ell_l}}(\varphi_{p-as-\ell_l}) = &
 \big(\neg(\exists wrkFor^-.o_e \equiv o_\nil)  \land
 \varphi_{p-as-\ell_l} \big) \lor \\
 &\exists wrkFor^-.o_e \equiv o_\nil\hphantom{)}\land
 \Psi_{e.wrkFor := proj}(\varphi_{p-as-\ell_l})\big)\\
\Psi_{e.wrkFor := proj}(\varphi_{p-as-\ell_l}) =&
 P_1 \sqcap\exists wrkFor_\gho.o_{\nil} \equiv  \\
 & P_1\sqcap\exists {((wrkFor\backslash (o_{e} \times \top)) \cup (o_e,o_{proj}))}.o_{proj}
\end{array}
\]
$\Psi_{e.wrkFor := proj}(\varphi_{p-as-\ell_l})$ is obtained from $\varphi_{p-as-\ell_l}$ by substituting the $wrkFor$
role with the correction  $((wrkFor\backslash (o_{e} \times \top)) \cup (o_e,o_{proj}))$
which updates the value of $o_e$ in $wrkFor$ to $proj$.
$\Phi_{S_{\ell_l}}(\varphi_{p-as-\ell_l})$ is obtained from $\Psi_{S_{\ell_l}}(\varphi_{p-as-\ell_l})$
by subtituting ${P_1}$ with ${P_1}^{ext}$.
$\Theta$ is differs from $\Phi$ from technical reasons related to
aborting computations (see Appendix \ref{app:backward}).
%
% \setcounter{tocdepth}{4}
% \tableofcontents
%

 \input{appendix-backwards}


